Delocalization of two-dimensional random surfaces with hard-core constraints

We study the fluctuations of random surfaces on a two-dimensional discrete torus. The random surfaces we consider are defined via a nearest-neighbor pair potential which we require to be twice continuously differentiable on a (possibly infinite) interval and infinity outside of this interval. No convexity assumption is made and we include the case of the so-called hammock potential, when the random surface is uniformly chosen from the set of all surfaces satisfying a Lipschitz constraint. Our main result is that these surfaces delocalize, having fluctuations whose variance is at least of order $\log n$, where $n$ is the side length of the torus. We also show that the expected maximum of such surfaces is of order at least $\log n$. The main tool in our analysis is an adaptation to the lattice setting of an algorithm of Richthammer, who developed a variant of a Mermin-Wagner-type argument applicable to hard-core constraints. We rely also on the reflection positivity of the random surface model. The result answers a question mentioned by Brascamp, Lieb and Lebowitz 1975 on the hammock potential and a question of Velenik 2006.

==> pictures.tex <==
 \newcommand{\scT}{0.4}
   

\begin{adjustwidth}{-1.0cm}{}   

%\begin{table}
 %        \caption {Table Title}
\begin{tabular}{|c|c|c|}    
%	\hline
    \multicolumn{3}{c}{Table 1: An illustration of the action of the addition algorithm on a function defined on a 2x3 grid graph.}\\
\hline 
\begin{sideways}
\parbox{6cm}{
 \underline{Initialization.} The vertices are assigned initial requested shifts, $\tau_1:=\tau$.
\newline\newline 
\underline{Loop } 
\begin{enumerate}
	\item[(1)] The green (gray in b\&w) vertex is set to be $P_1$ and to be processed.
	\item[(2)] It is shifted by $s_1 := 0$.
	\item[(3)] The requested shifts are updated. In this example for all $w$: $\tau_2(w,\varphi_w) := \tau_1(w,\varphi_w)$.
\end{enumerate}

}      $\:$       
\end{sideways} &
\begin{sideways}
\parbox{6cm}{
 	\underline{Loop } 
	\begin{enumerate}
		\item[(1)] The green (gray in b\&w)  vertex is set to be $P_2$ and to be processed.
		\item[(2)] It is shifted by $s_2 := 0.2$.
		\item[(3)] The requested shifts are updated. For the top-most vertex $v$: {\small $\tau_3(v,\varphi_v):=0.6<1.1=\tau_2(v,\varphi_v)$.} For all other $w$:   $\tau_3(w,\varphi_w) := \tau_2(w,\varphi_w)$.
	\end{enumerate}  
	{\small The next vertex to be processed need not be adjacent to the previously processed vertices.}
}   
\end{sideways}
  & 
\begin{sideways}
\parbox{6cm}{
   	\underline{Loop } 
	\begin{enumerate}
		\item[(1)] The green (gray in b\&w)  vertex is set to be $P_3$ and to be processed.
		\item[(2)] It is shifted by $s_3 := 0.3$.
		\item[(3)] The requested shifts are updated. For the top-center vertex $v$: {\small $\tau_4(v,\varphi_v):=0.69<1.2=\tau_3(v,\varphi_v)$.} For all other $w$:   $\tau_4(w,\varphi_w) := \tau_3(w,\varphi_w)$.
	\end{enumerate}
}
\end{sideways}

\tabularnewline
\hline 
\includegraphics[angle=90,scale=\scT]{pic1c} & \includegraphics[angle=90,scale=\scT]{pic2cBis.pdf} & \includegraphics[angle=90,scale=\scT]{pic3cBis.pdf}\\
\hline
\includegraphics[angle=90,scale=\scT]{pic1b} & \includegraphics[angle=90,scale=\scT]{pic2b.pdf} & \includegraphics[angle=90,scale=\scT]{pic3b.pdf}\\
\hline
\includegraphics[angle=90,scale=\scT]{pic1a} & \includegraphics[angle=90,scale=\scT]{pic2a.pdf} & \includegraphics[angle=90,scale=\scT]{pic3a.pdf}\\
\hline 
\end{tabular}
%\end{table}
\newpage 
\begin{tabular}{|c|c|c|}
%\hline              
   \multicolumn{3}{c}{Table 1: An illustration of the action of the addition algorithm (cont.)} \\
\hline
\begin{sideways}
\parbox{6cm}{
 	\underline{Loop } 
	\begin{enumerate}
		\item[(1)] The green (gray in b\&w)  vertex is set to be $P_4$ and to be processed.
		\item[(2)] It is shifted by $s_4 := 0.35$.
		\item[(3)] The requested shifts are updated. For the top-center vertex $v$: {\small $\tau_5(v,\varphi_v):=0.5<0.69=\tau_4(v,\varphi_v)$.} For all other $w$:   $\tau_5(w,\varphi_w) := \tau_4(w,\varphi_w)$.
	\end{enumerate}   
	{\small The requested shift of a vertex may be decreased several times.}

}   $\:$       
\end{sideways} &
\begin{sideways}
\parbox{6cm}{
 	 \underline{Loop } 
		\begin{enumerate}
			\item[(1)] The green (gray in b\&w)  vertex is set to be $P_5$ and to be processed.
			\item[(2)] It is shifted by $s_5 := 0.5$.
			\item[(3)] The requested shifts are updated. For the top-left vertex $v$: {\small $\tau_6(v,\varphi_v):=0.55<0.6=\tau_5(v,\varphi_v)$.} For the processed vertices (all except $v$) $\tau_6:=\tau_5$.
		\end{enumerate}  
}
\end{sideways}
  & 
\begin{sideways}
\parbox{6cm}{
   	 \underline{Loop } 
		\begin{enumerate}
			\item[(1)] The green (gray in b\&w)  vertex is set to be $P_6$ and to be processed.
			\item[(2)] It is shifted by $s_6 := 0.55$.
		\end{enumerate}  
		\vspace{2pt}
		{\small  The consecutive shifts increase, \\$s_1 \leq s_2 \leq s_3 \leq s_4\leq s_5 \leq s_6.$\\}
		{~\\}
		\begin{center}
			The algorithm terminates!
		\end{center}
}
\end{sideways}

\tabularnewline
\hline 
\includegraphics[angle=90,scale=\scT]{pic4cBis.pdf} & \includegraphics[angle=90,scale=\scT]{pic5cBis.pdf} & \includegraphics[angle=90,scale=\scT]{pic6c.pdf}\\
\hline
\includegraphics[angle=90,scale=\scT]{pic4b} & \includegraphics[angle=90,scale=\scT]{pic5b.pdf} & \includegraphics[angle=90,scale=\scT]{pic6b.pdf}\\
\hline
\includegraphics[angle=90,scale=\scT]{pic4a} & \includegraphics[angle=90,scale=\scT]{pic5a.pdf} & \includegraphics[angle=90,scale=\scT]{pic6a.pdf}\\
\hline 
\end{tabular}   
  \end{adjustwidth}
